A Distributed Flexible Delay-tolerant Proximal Gradient Algorithm

We develop and analyze an asynchronous algorithm for distributed convex optimization when the objective writes a sum of smooth functions, local to each worker, and a non-smooth function. Unlike many existing methods, our distributed algorithm is adjustable to various levels of communication cost, delays, machines computational power, and functions smoothness. A unique feature is that the stepsizes do not depend on communication delays nor number of machines, which is highly desirable for scalability. We prove that the algorithm converges linearly in the strongly convex case, and provide guarantees of convergence for the non-strongly convex case. The obtained rates are the same as the vanilla proximal gradient algorithm over some introduced epoch sequence that subsumes the delays of the system. We provide numerical results on large-scale machine learning problems to demonstrate the merits of the proposed method.

==> Figs/delays.tex <==


\begin{figure}
    \centering
    \begin{subfigure}{\columnwidth}
    \centering
     \begin{tikzpicture}[scale=0.5]
     %%% BASE
    \draw[thick, ->] (0,0) -- (10,0) node [below] {global time};
    \foreach \x in {1,...,19}
    \draw (\x/2, 0.1) -- node[pos=0.5] (point\x) {} (\x/2.0, -0.1);
    

    \draw (0,1.8) -- (0,3.2) -- (10.5,3.2) -- (10.5,1.8) -- (0,1.8);
    \node[draw,diamond,aspect=0.5,fill=gray!50!white, scale = 0.4] at (0.5,2.5) {$\Delta_i$};
    \node at (2.8,2.5) {~ updates of $i$};
    \node[draw,circle,fill=red, scale = 0.8] (B) at (6.5,2.5) {};
    \node at (8.45,2.5) {~ iteration $k$};
    
    %%%% Specific
    \node[draw,diamond,aspect=0.5,fill=gray!50!white, scale = 0.4] (B) at (7.5,0) {$\Delta_i$};
    \node[draw,circle,fill=red, scale = 0.8]  at (7.5,0) {};
    \node[scale=0.8] at (7.5,-0.95) {$k$};
    \node[draw,diamond,aspect=0.5,fill=gray!50!white, scale = 0.4] (B) at (5,0) {$\Delta_i$};
    \node[scale=0.8] at (5,-0.95) {$k-D_i^k$};
    \node[draw,diamond,aspect=0.5,fill=gray!50!white, scale = 0.4] (B) at (2.5,0) {$\Delta_i$};
    \node[draw,diamond,aspect=0.5,fill=gray!50!white, scale = 0.4] (B) at (1.5,0) {$\Delta_i$};
    
  \end{tikzpicture}
  \caption{$i=i(k)$ ~~~ ($d_i^k=0$)}
  \end{subfigure}\\[0.5cm]
      \begin{subfigure}{\columnwidth}
      \centering
     \begin{tikzpicture}[scale=0.5]
     %%% BASE
    \draw[thick, ->] (0,0) -- (10,0) node [below] {global time};
    \foreach \x in {1,...,19}
    \draw (\x/2, 0.1) -- node[pos=0.5] (point\x) {} (\x/2.0, -0.1);
    

    
    %%%% Specific
    \node[draw,circle,fill=red, scale = 0.8]  at (7.5,0) {};
    \node[scale=0.8] at (7.5,-0.95) {$k$};
    \node[draw,diamond,aspect=0.5,fill=gray!50!white, scale = 0.4] (B) at (6.0,0) {$\Delta_i$};
    \node[scale=0.8] at (6,-0.95) {$k-d_i^k$};
    \node[draw,diamond,aspect=0.5,fill=gray!50!white, scale = 0.4] (B) at (3.5,0) {$\Delta_i$};
    \node[scale=0.8] at (3.5,-0.95) {$k-D_i^k$};
    \node[draw,diamond,aspect=0.5,fill=gray!50!white, scale = 0.4] (B) at (2.0,0) {$\Delta_i$};
    \node[draw,diamond,aspect=0.5,fill=gray!50!white, scale = 0.4] (B) at (0.5,0) {$\Delta_i$};
    
  \end{tikzpicture}
  \caption{$i\neq i(k)$ ~~~ ($d_i^k>0$)}
  \end{subfigure}
  
    \caption{Illustration of the delays notation.}
    \label{fig:delays}
\end{figure}


==> num_res/strong.tex <==
\begin{tikzpicture}[scale=1]
\begin{groupplot}[group style={group name=plot2, group size= 2 by 1},width=\textwidth]

\nextgroupplot[ 
 width=0.45\columnwidth, 
 height=0.3\columnwidth, 
 xmin=0, 
 xmax = 7000,
 xmajorgrids, 
ymode=log,
 yminorticks=true, 
 ymajorgrids, 
 yminorgrids, 
 ylabel={Suboptimality },
 xlabel={Wallclock time (s)},
 %x label style={at={(axis description cs:0.5,-0.05)},anchor=north},
 ]




 \addplot [  each nth point=3, filter discard warning=false, unbounded coords=discard, 
 color=blue, 
 solid, 
 line width=2.0pt, 
 mark size=2.5pt, 
 mark=none
 ] 
file {  num_res/kdda/dave_rpg.csv };
 \label{plots1:dave}


 \addplot [  each nth point=3, filter discard warning=false, unbounded coords=discard, 
 color=gray, 
 solid, 
 line width=2.0pt, 
 mark size=2.5pt, 
 mark=none,
 ] 
file {  num_res/kdda/synch_gd.csv };
 \label{plots1:gd}

 \addplot [  each nth point=3, filter discard warning=false, unbounded coords=discard, 
 color=green!40!black, 
 solid, 
 line width=2.0pt, 
 mark size=2.5pt, 
 mark=none
 ] 
file {  num_res/kdda/piag.csv };
 \label{plots1:piag}



\nextgroupplot[ 
 width=0.45\columnwidth, 
 height=0.3\columnwidth, 
xmin = 0,
xmax= 5000,
 xmajorgrids, 
 ymode=log,
 yminorticks=true, 
 ymajorgrids, 
 yminorgrids, 
 %ylabel={Functional error },
 xlabel={Wallclock time (s)},
 %x label style={at={(axis description cs:0.5,0.05)},anchor=north},
 ]





 \addplot [  each nth point=3, filter discard warning=false, unbounded coords=discard, 
 color=blue, 
 solid, 
 line width=2.0pt, 
 mark size=2.5pt, 
 mark=none
 ] 
file {  num_res/url/dave_rpg.csv };



 \addplot [  each nth point=3, filter discard warning=false, unbounded coords=discard, 
 color=gray, 
 solid, 
 line width=2.0pt, 
 mark size=2.5pt, 
 mark=none
 ] 
file {  num_res/url/synch_gd.csv };

 \addplot [  each nth point=3, filter discard warning=false, unbounded coords=discard, 
 color=green!50!black, 
 solid, 
 line width=2.0pt, 
 mark size=2.5pt, 
 mark=none
 ] 
file { num_res/url/piag.csv };



\end{groupplot}

\node[anchor=north] at ($(plot2 c1r1.south)+(0,-1.0)$) { (a) KDDA };
\node[anchor=north] at ($(plot2 c1r1.south)+(0,-1.4)$) { \footnotesize $m=8,407,752$, $\lambda_1=10^{-7}$, $\lambda_2=\frac{1}{m}$ };
\node[anchor=north] at ($(plot2 c2r1.south)+(0,-1.0)$) { (b) URL ($n=3,231,961$) };


% legend
\path (plot2 c1r1.north west|-current bounding box.north)--
      coordinate(legendpos)
      (plot2 c2r1.north east|-current bounding box.north);
\matrix[
    matrix of nodes,
    anchor=south,
    draw,
    inner sep=0.2em,
    draw
  ]at([yshift=1ex]legendpos)
  {
    \ref{plots1:dave}& \texttt{DAve-RPG} $p=1$ &[5pt]
\ref{plots1:gd}& Synchronous PG &[5pt]
\ref{plots1:piag}&   PIAG \\
};
\end{tikzpicture}


==> shared_article.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.


% Packages and macros go here
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{algorithmic}
\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

\usepackage{amssymb,amsmath,amsthm,amscd,amstext,bbm, enumerate, dsfont, mathtools}
\usepackage{array}
\usepackage{multicol}
\usepackage{multirow}
\usepackage[algo2e]{algorithm2e}
\usepackage{algorithm}
%\usepackage{caption}
\usepackage{subcaption}
\usepackage{graphicx}
\usepackage{hyperref}
\usepackage{tcolorbox}
\usepackage{import}
\usepackage{pifont}
\usepackage{tikz,pgfplots}
\usetikzlibrary{tikzmark,shapes}
\usetikzlibrary{matrix}
\usepgfplotslibrary{groupplots}






\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator*{\dom}{dom}
% \DeclareMathOperator*{\prox}{\mathrm{prox}}

\newcommand{\prox}{\mathop{\mathrm{prox}}\nolimits}
% \newcommand{\prox}{\text{prox}}
\newcommand{\Sum}{\sum\limits_{i=1}^M}
\newcommand{\Sumj}{\sum\limits_{j=1}^M}
%\newcommand{\pr}{\prox_{\gamma r}}
\newcommand{\EE}{\mathbb{E}}



\newcommand{\funi}{ \frac{1}{n_i} \sum_{j\in\mathcal{S}_i} \ell_j}
\newcommand{\nablafuni}{ \frac{1}{n_i} \sum_{j\in\mathcal{S}_i} \nabla \ell_j}


\newtheorem{innercustomthm}{Theorem}
\newenvironment{customthm}[1]
  {\renewcommand\theinnercustomthm{#1}\innercustomthm}
  {\endinnercustomthm}
  
\newtheorem{innercustomlem}{Lemma}
\newenvironment{customlem}[1]
  {\renewcommand\theinnercustomlem{#1}\innercustomlem}
  {\endinnercustomlem}
  



\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{corollary}{Corollary}
\newtheorem{coro}{Corollary}
\newtheorem{assumption}{Assumption}
\newtheorem{proposition}{Proposition}
\newtheorem*{remark}{Remark}

\numberwithin{coro}{section}



%strongly recommended
\numberwithin{theorem}{section}

% Declare title and authors, without \thanks
\newcommand{\TheTitle}{A Distributed Flexible Delay-tolerant Proximal Gradient Algorithm } 
\newcommand{\TheAuthors}{K. Mishchenko, F. Iutzeler, and J. Malick}

% Sets running headers as well as PDF title and authors
%\headers{\TheTitle}{\TheAuthors}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
\title{{\TheTitle}}
%\funding{This work was partially funded by ...}}}



% Authors: full names plus addresses.
\author{
  Konstantin Mishchenko\thanks{KAUST
    (\url{konstantin.mishchenko@kaust.edu.sa}, \url{http://konstmish.github.io/}).}
  \and
  Franck Iutzeler\thanks{Laboratoire Jean Kuntzmann, Univ. Grenoble Alpes (\url{franck.iutzeler@univ-grenoble-alpes.fr}).}
  \and
  J\'er\^{o}me Malick\thanks{CNRS, Laboratoire Jean Kuntzmann  (\url{jerome.malick@univ-grenoble-alpes.fr}).}
}

\usepackage{amsopn}
\DeclareMathOperator{\diag}{diag}



